AT2019azh: an unusually long-lived, radio-bright thermal tidal disruption event

Tidal disruption events (TDEs) occur when a star is destroyed by a supermassive black hole at the center of a galaxy, temporarily increasing the accretion rate onto the black hole and producing a bright flare across the electromagnetic spectrum. Radio observations of TDEs trace outflows and jets that may be produced. Radio detections of the outflows from TDEs are uncommon, with only about one third of TDEs discovered to date having published radio detections. Here we present over two years of comprehensive, multi-radio frequency monitoring observations of the tidal disruption event AT2019azh taken with the Very Large Array (VLA) and MeerKAT radio telescopes from approximately 10 days pre-optical peak to 810 days post-optical peak. AT2019azh shows unusual radio emission for a thermal TDE, as it brightened very slowly over two years, and showed fluctuations in the synchrotron energy index of the optically thin synchrotron emission from 450 days post-disruption. Based on the radio properties, we deduce that the outflow in this event is likely non-relativistic and could be explained by a spherical outflow arising from self-stream intersections, or a mildly collimated outflow from accretion onto the supermassive black hole. This data-set provides a significant contribution to the observational database of outflows from TDEs, including the earliest radio detection of a non-relativistic TDE to date, relative to the optical discovery.

==> obstable.tex <==
\begin{table*}
 \label{tab:radio_obs}
 \caption{Radio observations of AT2019azh taken with the VLA and MeerKAT. {\color{red}\textbf{Need to resolve argument with latex and make table multicolumn/run nicely over pages.}} }
 \newcolumntype{~}{!{\vrule width 0.5pt}}
 \begin{tabular}{p{0.4cm}p{2cm}p{0.4cm}p{0.5cm}p{0.5cm}p{0.5cm}p{0.5cm}p{0.5cm}p{0.6cm}}%~p{0.4cm}p{2cm}p{0.4cm}p{0.5cm}p{0.5cm}p{0.5cm}p{0.5cm}p{0.5cm}p{0.5cm}} 
    %\begin{longtable}{l{0.5cm}c{0.5cm}c{0.5cm}c{0.5cm}c{0.5cm}c{0.5cm}c{0.5cm}c{0.5cm}c{0.5cm}} 
        \hline
        Epoch & Date (UTC) & $\delta$t (d) &  Array&Config.& Band & $\nu$ (GHz) & $F_{\nu}$ ($\mu$Jy) & $u(F_{\nu})$ ($\mu$Jy) \\%Epoch & Date (UTC) & $\delta$t (d) &  Array&Config.& Band & $\nu$ (GHz) & $F_{\nu}$ ($\mu$Jy) & $u(F_{\nu})$ ($\mu$Jy)  \\
        % \endfirsthead
        % \endhead
        % \multicolumn{15}{r}{\footnotesize\itshape Continued on the next page}
        % \endfoot
        % \endlastfoot
        \hline
        \hline
        1 & 2019-03-09 1:10 & 29 & VLA & B & X & 10 & 150 & 12 \\
        \\
        2 & 2019-04-14 2:34 & 65 & VLA & B & K & 24 & 262 & 11 \\
         &  &  &  &  & X & 11 & 286 & 12 \\
         &  &  &  &  & X & 9 & 331 & 9 \\
         &  &  &  &  & C & 7.511 & 343 & 8 \\
         &  &  &  &  & C & 6.487 & 356 & 9 \\
         &  &  &  &  & C & 5.511 & 383 & 9 \\
         &  &  &  &  & C & 4.487 & 455 & 11 \\
        \\
        3 & 2019-05-12 20:39 & 94 & VLA & B & Ku & 14 & 233 & 8 \\
         &  &  &  &  & X & 11 & 258 & 10 \\
         &  &  &  &  & X & 9 & 320 & 10 \\
         &  &  &  &  & C & 7.5 & 360 & 9 \\
         &  &  &  &  & C & 6.5 & 362 & 10 \\
         &  &  &  &  & C & 5.5 & 375 & 9 \\
         &  &  &  &  & C & 4.5 & 434 & 10 \\
         \\
        4 & 2019-05-20 23:51 & 102 & VLA & B & C & 7.45 & 377 & 22 \\
         &  &  &  &  & C & 6.49 & 472 & 21 \\
         &  &  &  &  & C & 5.51 & 401 & 18 \\
         &  &  &  &  & C & 4.49 & 564 & 20 \\
         &  &  &  &  & S & 3.76 & 582 & 27 \\
         &  &  &  &  & S & 3.24 & 636 & 22 \\
         &  &  &  &  & S & 2.76 & 616 & 29 \\
         &  &  &  &  & S & 2.24 & 678 & 61 \\
         &  &  &  &  & L & 1.776 & 906 & 142 \\
         \\
        5 & 2019-06-19 23:40 & 132 & VLA & B & X & 10.999 & 306 & 12 \\
         &  &  &  &  & X & 8.999 & 355 & 12 \\
         &  &  &  &  & C & 7.511 & 454 & 14 \\
         &  &  &  &  & C & 6.487 & 484 & 14 \\
         &  &  &  &  & C & 5.511 & 522 & 15 \\
         &  &  &  &  & C & 4.487 & 645 & 19 \\
         &  &  &  &  & S & 3.755 & 617 & 20 \\
         &  &  &  &  & S & 3.243 & 677 & 18 \\
         &  &  &  &  & S & 2.755 & 801 & 21 \\
         &  &  &  &  & S & 2.243 & 798 & 37 \\
         &  &  &  &  & L & 1.903 & 933 & 42 \\
         &  &  &  &  & L & 1.648 & 945 & 53 \\
         &  &  &  &  & L & 1.3916 & 1195 & 38 \\
         &  &  &  &  & L & 1.136 & 1240 & 160 \\
         \\
        6 & 2019-08-09 19:06 & 183& VLA & A & X & 11 & 346 & 12 \\
         &  &  &  &  & X & 9 & 450 & 11 \\
         &  &  &  &  & C & 7.511 & 526 & 13 \\
         &  &  &  &  & C & 6.487 & 593 & 15 \\
         &  &  &  &  & C & 5.511 & 707 & 14 \\
         &  &  &  &  & C & 4.487 & 824 & 15 \\
         &  &  &  &  & S & 3.755 & 867 & 18 \\
         &  &  &  &  & S & 3.243 & 1002 & 17 \\
         &  &  &  &  & S & 2.755 & 1069 & 19 \\
         &  &  &  &  & S & 2.243 & 1175 & 46 \\
         &  &  &  &  & L & 1.9035 & 1164 & 43 \\
         &  &  &  &  & L & 1.6475 & 1190 & 68 \\
         &  &  &  &  & L & 1.3915 & 1306 & 38 \\
         &  &  &  &  & L & 1.1355 & 1217 & 88 \\
        \\
        7 & 2019-10-19 15:04 & 254& VLA & A & X & 11 & 382 & 9 \\
         &  &  &  &  & X & 9 & 483 & 9 \\
         &  &  &  &  & S & 3.755 & 1128 & 16 \\
         &  &  &  &  & S & 3.243 & 1234 & 15 \\
         &  &  &  &  & S & 2.755 & 1360 & 17 \\
         &  &  &  &  & S & 2.243 & 1518 & 26 \\
         &  &  &  &  & L & 1.9035 & 1612 & 34 \\
         &  &  &  &  & L & 1.6475 & 1737 & 60 \\
         &  &  &  &  & L & 1.3915 & 1762 & 31 \\
         &  &  &  &  & L & 1.1355 & 1717 & 51 \\
         \\
         & 2019-11-25 1:02 &  & MeerKAT &  & L & 1.284 & 1990 & 40 \\
         \\
        8 & 2019-11-30 12:32 & 296 & VLA & D & X & 11 & 580 & 23 \\
         &  &  &  &  & X & 9 & 672 & 24 \\
         &  &  &  &  & S & 3.627 & 1870 & 360 \\
         &  &  &  &  & S & 3.243 & 1515 & 33 \\
         &  &  &  &  & S & 2.755 & 1620 & 36 \\
         &  &  &  &  & S & 2.243 & 1760 & 150 \\
         \\
         & 2020-01-29 21:50 &  & MeerKAT &  & L & 1.284 & 2121 & 42 \\
         \\
        9 & 2020-01-24 9:27 & 350 & VLA & D & X & 11 & 889 & 24 \\
         &  &  &  &  & X & 9 & 979 & 21 \\
         &  &  &  &  & S & 3.755 & 1817 & 37 \\
         &  &  &  &  & S & 3.24 & 1876 & 35 \\
         &  &  &  &  & S & 2.76 & 1886 & 45 \\
         &  &  &  &  & S & 2.243 & 2300 & 130 \\
         \\
         & 2020-05-05 15:08 &  & MeerKAT &  & L & 1.284 & 4311 & 86 \\
         \\
        10 & 2020-05-11 22:19 & 459 & VLA & C & X & 11 & 595 & 12 \\
         &  &  &  &  & X & 9 & 836 & 11 \\
         &  &  &  &  & C & 4.487 & 1953 & 16 \\
         &  &  &  &  & C & 5.511 & 1550 & 18 \\
         &  &  &  &  & C & 6.487 & 1293 & 20 \\
         &  &  &  &  & C & 7.511 & 1098 & 15 \\
         &  &  &  &  & S & 2.243 & 3703 & 62 \\
         &  &  &  &  & S & 2.755 & 3306 & 22 \\
         &  &  &  &  & S & 3.243 & 2818 & 20 \\
         &  &  &  &  & S & 3.755 & 2306 & 31 \\
         \\
        & 2020-11-14 4:40 &  & MeerKAT &  & L & 1.284 & 4460 & 89 \\
         \\
        11 & 2020-12-05 08:02 & 666 & VLA & bnA->A & X & 10.999 & 1063.6 & 8 \\
         &  &  &  &  & X & 8.999 & 1328.3 & 7.8 \\
         &  &  &  &  & C & 7.511 & 1573 & 14 \\
         &  &  &  &  & C & 6.487 & 1802 & 16 \\
         &  &  &  &  & C & 5.511 & 2163 & 19 \\
         &  &  &  &  & C & 4.487 & 2458 & 17 \\
         &  &  &  &  & S & 3.754 & 2798 & 25 \\
         &  &  &  &  & S & 3.243 & 3022 & 26 \\
         &  &  &  &  & S & 2.754 & 3321 & 34 \\
         &  &  &  &  & S & 2.243 & 3679 & 41 \\
         &  &  &  &  & L & 1.903 & 3960 & 44 \\
         &  &  &  &  & L & 1.6474 & 4197 & 41 \\
         &  &  &  &  & L & 1.391 & 4454 & 44 \\
         &  &  &  &  & L & 1.135 & 4610 & 120 \\
         &  &  &  &  & P & 0.352 & 2100 & 1000 \\
         \\
        12 & 2021-02-26 07:03 & 749 & VLA & A & X & 11 & 677.3 & 8.4 \\
         &  &  &  &  & X & 9 & 904 & 8.3 \\
         &  &  &  &  & C & 7.51 & 1081 & 14 \\
         &  &  &  &  & C & 6.488 & 1263 & 17 \\
         &  &  &  &  & C & 5.512 & 1505 & 19 \\
         &  &  &  &  & C & 4.487 & 1912 & 16 \\
         &  &  &  &  & S & 3.76 & 2306 & 23 \\
         &  &  &  &  & S & 3.24 & 2659 & 23 \\
         &  &  &  &  & S & 2.755 & 3101 & 26 \\
         &  &  &  &  & S & 2.243 & 3782 & 57 \\
         &  &  &  &  & L & 1.9 & 4251 & 29 \\
         &  &  &  &  & L & 1.39 & 5410 & 32 \\
         &  &  &  &  & P & 0.351 & 4600 & 1700 \\
        \\
        13 & 2021-05-06 20:02 & 849 & VLA & D->C & X & 11 & 543 & 43 \\
       &  &  &  &  &  X	&9	&598&	36\\
        &  &  &  &  & C	&7.51&	682	&39\\
        &  &  &  &  & C	&6.49&	806	&28\\
        &  &  &  &  & C	&5.51&	1035&	39\\
        &  &  &  &  & C	&4.49&	1293&	43\\
        &  &  &  &  & S	&3.76&	1520&	35\\
        &  &  &  &  & S	&2.371&	1783&	63\\
        &  &  &  &  & L	&1.77&	2407&	60\\
        &  &  &  &  & L	&1.36&	2440&	100\\
        
        \hline
    \end{tabular}
    \textbf{Notes:} $\delta t$ is measured with reference to the estimated outflow launch date, $t_0=$ MJD\,58522.
\end{table*}
%%%%%%%%%%%%%%%%%%%% end data table %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
